Domain-Specific Latent Representations Improve the Fidelity of Diffusion-Based Medical Image Super-Resolution

Latent diffusion models for medical image super-resolution universally inherit variational autoencoders designed for natural photographs. We show that this default choice, not the diffusion architecture, is the dominant constraint on reconstruction quality. In a controlled experiment holding all other pipeline components fixed, replacing the generic Stable Diffusion VAE with MedVAE, a domain-specific autoencoder pretrained on more than 1.6 million medical images, yields +2.91 to +3.29 dB PSNR improvement across knee MRI, brain MRI, and chest X-ray (n = 1,820; Cohen's d = 1.37 to 1.86, all p < 10^{-20}, Wilcoxon signed-rank). Wavelet decomposition localises the advantage to the finest spatial frequency bands encoding anatomically relevant fine structure. Ablations across inference schedules, prediction targets, and generative architectures confirm the gap is stable within plus or minus 0.15 dB, while hallucination rates remain comparable between methods (Cohen's h < 0.02 across all datasets), establishing that reconstruction fidelity and generative hallucination are governed by independent pipeline components. These results provide a practical screening criterion: autoencoder reconstruction quality, measurable without diffusion training, predicts downstream SR performance (R^2 = 0.67), suggesting that domain-specific VAE selection should precede diffusion architecture search. Code and trained model weights are publicly available at https://github.com/sebasmos/latent-sr.

==> shortcut_ontology_v2.tex <==
% shortcut_ontology_v2.tex  –  TikZ-free version of the unified ontology figure
% Include from main.tex with:  \input{figures/shortcut_ontology_v2}
%
% Requires only: xcolor, soul, tabularx (already loaded by main.tex)

\begin{figure*}[!tb]
\centering

% ── ROOT: Unified Definition ──────────────────────────────────────
\fcolorbox{black!60}{black!80}{%
\parbox{0.88\textwidth}{\centering\color{white}%
  {\scriptsize\sffamily\bfseries UNIFIED DEFINITION}\\[2pt]
  {\large\bfseries SHORTCUT}\\[4pt]
  {\small\itshape A compressed decision rule that exploits environmental regularity to reduce processing cost.\\
  Substrate-neutral.\ Adaptive when environment-matched and causally grounded;\\
  harmful when mismatched or spuriously correlated.}%
}}

\vspace{6pt}
{\color{gray!50}\rule{0.4pt}{10pt}}% vertical connector
\vspace{2pt}

% ── SHARED PROPERTIES ─────────────────────────────────────────────
\fcolorbox{orange!40}{orange!5}{%
\parbox{0.88\textwidth}{\centering
  {\scriptsize\sffamily\bfseries\color{orange!70!black} SHARED PROPERTIES}\\[4pt]
  Compression \quad$\cdot$\quad Resource reduction \quad$\cdot$\quad Heuristic \quad$\cdot$\quad Environment-dependent validity \quad$\cdot$\quad Minimum-cost optimization%
}}

\vspace{6pt}

% ── TWO BRANCHES ──────────────────────────────────────────────────
\noindent
\begin{minipage}[t]{0.47\textwidth}
\centering
% branch header
\fcolorbox{teal!50}{teal!8}{%
\parbox{0.95\linewidth}{\centering
  {\sffamily\bfseries\color{teal!70!black} Biological / Cultural}\\
  {\scriptsize\color{gray} Evolved \& transmitted heuristics}%
}}

\vspace{4pt}
{\scriptsize
\begin{tabular}{@{}p{1.6cm}p{4.2cm}@{}}
\textbf{Medium}       & Neural tissue, cultural practice \\[1pt]
\textbf{Resource}     & Calories, cognitive load \\[1pt]
\textbf{Transmission} & Beliefs, storytelling, social learning \\[1pt]
\textbf{Timescale}    & One lifetime $\to$ many generations \\[1pt]
\textbf{Environment}  & Physical ecology, social structure \\[1pt]
\textbf{Detection}    & Ethnographic observation, experiment \\
\end{tabular}}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.47\textwidth}
\centering
% branch header
\fcolorbox{purple!50}{purple!5}{%
\parbox{0.95\linewidth}{\centering
  {\sffamily\bfseries\color{purple!70} Computational}\\
  {\scriptsize\color{gray} Learned \& propagated correlations}%
}}

\vspace{4pt}
{\scriptsize
\begin{tabular}{@{}p{1.6cm}p{4.2cm}@{}}
\textbf{Medium}       & Embedding space geometry \\[1pt]
\textbf{Resource}     & Computational load, loss minimization \\[1pt]
\textbf{Transmission} & Gradient descent, weight inheritance \\[1pt]
\textbf{Timescale}    & Training run $\to$ foundation model propagation \\[1pt]
\textbf{Environment}  & Training distribution, data ecology \\[1pt]
\textbf{Detection}    & Probes, clustering, statistics (\textit{ShortKit-ML}) \\
\end{tabular}}
\end{minipage}

\vspace{8pt}

% ── EVALUATION MATRIX ─────────────────────────────────────────────
\fcolorbox{teal!30}{white}{%
\parbox{0.88\textwidth}{%
  {\scriptsize\sffamily\bfseries\color{teal!70!black} EVALUATION AXES}
  \quad{\tiny\itshape\color{gray} Applicable across both substrates}\\[6pt]
  \centering
  \begin{tabular}{@{}r|p{4.5cm}|p{4.5cm}@{}}
   & \centering\textbf{Causal Regularity} & \centering\textbf{Spurious Regularity} \tabularnewline
  \hline
  \textbf{Env-Matched} &
    \textbf{Adaptive Shortcut}\newline
    {\scriptsize Ecologically rational heuristic. Legitimate prior. Clinically useful signal.} &
    \textbf{Lucky Shortcut}\newline
    {\scriptsize Right answer, wrong reason. Locally valid, causally unsupported.} \\
  \hline
  \textbf{Env-Mismatched} &
    \textbf{Transferred Risk}\newline
    {\scriptsize Valid mechanism, wrong context. Domain shift of a real signal.} &
    \textbf{Active Harm}\newline
    {\scriptsize Spurious + mismatched. Hospital markers across sites. WEIRD standards on non-WEIRD populations.} \\
  \end{tabular}%
}}

\caption{Unified shortcut ontology across biological and computational substrates. A shortcut is a compressed decision rule that exploits environmental regularity to reduce processing cost---substrate-neutral in deep structure, divergent in encoding medium, transmission mechanism, and detection method. The evaluation matrix (bottom) applies across both substrates: shortcut valence is determined by the interaction of causal grounding and environmental match. \textit{ShortKit-ML} operates in the computational branch; a full treatment spanning both substrates is the subject of forthcoming work.}
\label{fig:ontology}
\end{figure*}

